Bridging Domains with Approximately Shared Features

Multi-source domain adaptation aims to reduce performance degradation when applying machine learning models to unseen domains. A fundamental challenge is devising the optimal strategy for feature selection. Existing literature is somewhat paradoxical: some advocate for learning invariant features from source domains, while others favor more diverse features. To address the challenge, we propose a statistical framework that distinguishes the utilities of features based on the variance of their correlation to label $y$ across domains. Under our framework, we design and analyze a learning procedure consisting of learning approximately shared feature representation from source tasks and fine-tuning it on the target task. Our theoretical analysis necessitates the importance of learning approximately shared features instead of only the strictly invariant features and yields an improved population risk compared to previous results on both source and target tasks, thus partly resolving the paradox mentioned above. Inspired by our theory, we proposed a more practical way to isolate the content (invariant+approximately shared) from environmental features and further consolidate our theoretical findings.

==> figures/3_linear_probing.tex <==
\begin{tabular}{llllllllll}
\toprule
    &  &  & 0.100000 & 0.200000 & 0.400000 & 0.600000 & 0.800000 & 1.000000 & mean \\
dataset.name & dataset.target_envs & hue &  &  &  &  &  &  &  \\
\midrule
\multirow[t]{44}{*}{officehome} & \multirow[t]{11}{*}{0} & DANN & 0.4527 ± 0.0107 & 0.5984 ± 0.0109 & 0.6527 ± 0.0090 & 0.7111 ± 0.0054 & 0.7193 ± 0.0092 & 0.7177 ± 0.0087 & 0.6420 ± 0.0090 \\
    &  & DIWA & 0.5835 ± 0.0132 & 0.6675 ± 0.0097 & 0.7276 ± 0.0094 & 0.7358 ± 0.0082 & 0.7720 ± 0.0118 & 0.7909 ± 0.0048 & 0.7129 ± 0.0095 \\
    &  & ERM & 0.5745 ± 0.0105 & 0.6848 ± 0.0046 & 0.7243 ± 0.0107 & 0.7539 ± 0.0108 & 0.7827 ± 0.0082 & 0.7926 ± 0.0085 & 0.7188 ± 0.0089 \\
    &  & NUC\_0.01 & 0.4840 ± 0.0129 & 0.6543 ± 0.0043 & 0.7407 ± 0.0097 & 0.7934 ± 0.0136 & 0.8049 ± 0.0040 & 0.8165 ± 0.0062 & 0.7156 ± 0.0084 \\
    &  & NUC\_0.1 & 0.4733 ± 0.0072 & 0.6782 ± 0.0111 & 0.7687 ± 0.0117 & 0.8049 ± 0.0038 & 0.8132 ± 0.0062 & 0.8099 ± 0.0077 & 0.7247 ± 0.0080 \\
    &  & PN\_B & 0.5852 ± 0.0051 & 0.6733 ± 0.0115 & 0.7449 ± 0.0068 & 0.7613 ± 0.0065 & 0.8165 ± 0.0025 & 0.8074 ± 0.0053 & 0.7314 ± 0.0063 \\
    &  & PN\_B-Y & 0.5770 ± 0.0076 & 0.6955 ± 0.0050 & 0.7490 ± 0.0068 & 0.7761 ± 0.0053 & 0.8074 ± 0.0094 & 0.8329 ± 0.0074 & 0.7396 ± 0.0069 \\
    &  & PN\_B-Y-S-E & 0.5844 ± 0.0057 & 0.7119 ± 0.0114 & 0.7366 ± 0.0077 & 0.7580 ± 0.0054 & 0.8041 ± 0.0110 & 0.8337 ± 0.0055 & 0.7381 ± 0.0078 \\
    &  & PN\_Y & 0.5877 ± 0.0080 & 0.7169 ± 0.0081 & 0.7481 ± 0.0102 & 0.7588 ± 0.0083 & 0.8066 ± 0.0075 & 0.8280 ± 0.0126 & 0.7410 ± 0.0091 \\
    &  & PN\_Y-S & 0.5745 ± 0.0070 & 0.7062 ± 0.0095 & 0.7432 ± 0.0135 & 0.7860 ± 0.0135 & 0.8041 ± 0.0127 & 0.8222 ± 0.0080 & 0.7394 ± 0.0107 \\
    &  & PN\_Y-S-E & 0.5901 ± 0.0098 & 0.7029 ± 0.0105 & 0.7498 ± 0.0068 & 0.7778 ± 0.0066 & 0.8082 ± 0.0028 & 0.8296 ± 0.0094 & 0.7431 ± 0.0077 \\
\cline{2-10}
    & \multirow[t]{11}{*}{1} & DANN & 0.4842 ± 0.0128 & 0.5986 ± 0.0077 & 0.6856 ± 0.0078 & 0.7011 ± 0.0090 & 0.7263 ± 0.0047 & 0.7318 ± 0.0072 & 0.6546 ± 0.0082 \\
    &  & DIWA & 0.5716 ± 0.0082 & 0.6577 ± 0.0101 & 0.7121 ± 0.0077 & 0.7487 ± 0.0067 & 0.7808 ± 0.0050 & 0.7725 ± 0.0082 & 0.7072 ± 0.0077 \\
    &  & ERM & 0.5538 ± 0.0071 & 0.6490 ± 0.0065 & 0.6989 ± 0.0054 & 0.7204 ± 0.0034 & 0.7432 ± 0.0038 & 0.7803 ± 0.0089 & 0.6909 ± 0.0058 \\
    &  & NUC\_0.01 & 0.4838 ± 0.0070 & 0.6293 ± 0.0049 & 0.6879 ± 0.0055 & 0.7414 ± 0.0075 & 0.7730 ± 0.0063 & 0.7867 ± 0.0053 & 0.6837 ± 0.0061 \\
    &  & NUC\_0.1 & 0.4824 ± 0.0101 & 0.6449 ± 0.0066 & 0.6728 ± 0.0095 & 0.7382 ± 0.0087 & 0.7744 ± 0.0061 & 0.7794 ± 0.0067 & 0.6820 ± 0.0080 \\
    &  & PN\_B & 0.5542 ± 0.0082 & 0.6568 ± 0.0028 & 0.7281 ± 0.0062 & 0.7684 ± 0.0059 & 0.7812 ± 0.0063 & 0.7973 ± 0.0026 & 0.7143 ± 0.0053 \\
    &  & PN\_B-Y & 0.5593 ± 0.0092 & 0.6545 ± 0.0035 & 0.7465 ± 0.0045 & 0.7808 ± 0.0092 & 0.7844 ± 0.0053 & 0.8009 ± 0.0064 & 0.7211 ± 0.0064 \\
    &  & PN\_B-Y-S-E & 0.5712 ± 0.0066 & 0.6526 ± 0.0076 & 0.7217 ± 0.0060 & 0.7698 ± 0.0060 & 0.7863 ± 0.0009 & 0.8064 ± 0.0044 & 0.7180 ± 0.0052 \\
    &  & PN\_Y & 0.5584 ± 0.0052 & 0.6563 ± 0.0068 & 0.7245 ± 0.0070 & 0.7817 ± 0.0058 & 0.7826 ± 0.0128 & 0.8018 ± 0.0056 & 0.7175 ± 0.0072 \\
    &  & PN\_Y-S & 0.5744 ± 0.0113 & 0.6517 ± 0.0025 & 0.7263 ± 0.0046 & 0.7744 ± 0.0070 & 0.7826 ± 0.0071 & 0.7899 ± 0.0092 & 0.7166 ± 0.0070 \\
    &  & PN\_Y-S-E & 0.5707 ± 0.0078 & 0.6613 ± 0.0035 & 0.7359 ± 0.0047 & 0.7661 ± 0.0034 & 0.7808 ± 0.0085 & 0.7995 ± 0.0030 & 0.7191 ± 0.0052 \\
\cline{2-10}
    & \multirow[t]{11}{*}{2} & DANN & 0.6649 ± 0.0056 & 0.7423 ± 0.0018 & 0.8230 ± 0.0062 & 0.8509 ± 0.0058 & 0.8667 ± 0.0036 & 0.8784 ± 0.0049 & 0.8044 ± 0.0046 \\
    &  & DIWA & 0.7734 ± 0.0082 & 0.8189 ± 0.0059 & 0.8649 ± 0.0049 & 0.8959 ± 0.0036 & 0.9063 ± 0.0052 & 0.9045 ± 0.0055 & 0.8607 ± 0.0055 \\
    &  & ERM & 0.7743 ± 0.0069 & 0.8401 ± 0.0019 & 0.8716 ± 0.0048 & 0.9113 ± 0.0038 & 0.8995 ± 0.0039 & 0.9122 ± 0.0033 & 0.8682 ± 0.0041 \\
    &  & NUC\_0.01 & 0.7176 ± 0.0030 & 0.8320 ± 0.0049 & 0.9077 ± 0.0031 & 0.9126 ± 0.0046 & 0.9261 ± 0.0024 & 0.9302 ± 0.0028 & 0.8710 ± 0.0035 \\
    &  & NUC\_0.1 & 0.7257 ± 0.0085 & 0.8279 ± 0.0052 & 0.8977 ± 0.0052 & 0.9198 ± 0.0032 & 0.9212 ± 0.0053 & 0.9248 ± 0.0023 & 0.8695 ± 0.0050 \\
    &  & PN\_B & 0.7689 ± 0.0024 & 0.8365 ± 0.0037 & 0.8689 ± 0.0053 & 0.8919 ± 0.0026 & 0.9140 ± 0.0034 & 0.9203 ± 0.0038 & 0.8667 ± 0.0035 \\
    &  & PN\_B-Y & 0.7721 ± 0.0083 & 0.8351 ± 0.0044 & 0.8613 ± 0.0039 & 0.8955 ± 0.0044 & 0.9144 ± 0.0034 & 0.9117 ± 0.0039 & 0.8650 ± 0.0047 \\
    &  & PN\_B-Y-S-E & 0.7797 ± 0.0038 & 0.8459 ± 0.0051 & 0.8730 ± 0.0039 & 0.8914 ± 0.0049 & 0.9162 ± 0.0008 & 0.9185 ± 0.0041 & 0.8708 ± 0.0038 \\
    &  & PN\_Y & 0.7527 ± 0.0071 & 0.8446 ± 0.0054 & 0.8770 ± 0.0042 & 0.8923 ± 0.0046 & 0.8991 ± 0.0060 & 0.9234 ± 0.0052 & 0.8649 ± 0.0054 \\
    &  & PN\_Y-S & 0.7703 ± 0.0074 & 0.8468 ± 0.0065 & 0.8671 ± 0.0033 & 0.8955 ± 0.0034 & 0.9027 ± 0.0039 & 0.9176 ± 0.0021 & 0.8667 ± 0.0044 \\
    &  & PN\_Y-S-E & 0.7770 ± 0.0069 & 0.8455 ± 0.0090 & 0.8829 ± 0.0074 & 0.8959 ± 0.0053 & 0.9023 ± 0.0054 & 0.9225 ± 0.0027 & 0.8710 ± 0.0061 \\
\cline{2-10}
    & \multirow[t]{11}{*}{3} & DANN & 0.6385 ± 0.0043 & 0.7183 ± 0.0051 & 0.7518 ± 0.0067 & 0.7638 ± 0.0044 & 0.7853 ± 0.0067 & 0.7862 ± 0.0058 & 0.7407 ± 0.0055 \\
    &  & DIWA & 0.7867 ± 0.0085 & 0.8000 ± 0.0034 & 0.8271 ± 0.0040 & 0.8408 ± 0.0044 & 0.8344 ± 0.0037 & 0.8560 ± 0.0073 & 0.8242 ± 0.0052 \\
    &  & ERM & 0.8248 ± 0.0050 & 0.8367 ± 0.0053 & 0.8619 ± 0.0044 & 0.8555 ± 0.0079 & 0.8546 ± 0.0084 & 0.8555 ± 0.0054 & 0.8482 ± 0.0061 \\
    &  & NUC\_0.01 & 0.7156 ± 0.0052 & 0.8147 ± 0.0085 & 0.8596 ± 0.0033 & 0.8670 ± 0.0036 & 0.8656 ± 0.0049 & 0.8812 ± 0.0112 & 0.8339 ± 0.0061 \\
    &  & NUC\_0.1 & 0.7165 ± 0.0111 & 0.8165 ± 0.0058 & 0.8587 ± 0.0017 & 0.8679 ± 0.0049 & 0.8624 ± 0.0030 & 0.8771 ± 0.0078 & 0.8332 ± 0.0057 \\
    &  & PN\_B & 0.7894 ± 0.0077 & 0.8312 ± 0.0036 & 0.8628 ± 0.0029 & 0.8651 ± 0.0031 & 0.8693 ± 0.0062 & 0.8633 ± 0.0066 & 0.8469 ± 0.0050 \\
    &  & PN\_B-Y & 0.7940 ± 0.0058 & 0.8252 ± 0.0023 & 0.8615 ± 0.0006 & 0.8656 ± 0.0034 & 0.8817 ± 0.0071 & 0.8647 ± 0.0039 & 0.8488 ± 0.0038 \\
    &  & PN\_B-Y-S-E & 0.7872 ± 0.0066 & 0.8353 ± 0.0099 & 0.8587 ± 0.0034 & 0.8633 ± 0.0039 & 0.8683 ± 0.0064 & 0.8665 ± 0.0060 & 0.8466 ± 0.0060 \\
    &  & PN\_Y & 0.7986 ± 0.0037 & 0.8422 ± 0.0074 & 0.8495 ± 0.0051 & 0.8615 ± 0.0046 & 0.8688 ± 0.0022 & 0.8720 ± 0.0028 & 0.8488 ± 0.0043 \\
    &  & PN\_Y-S & 0.7812 ± 0.0038 & 0.8381 ± 0.0030 & 0.8679 ± 0.0060 & 0.8628 ± 0.0039 & 0.8693 ± 0.0061 & 0.8835 ± 0.0028 & 0.8505 ± 0.0043 \\
    &  & PN\_Y-S-E & 0.7904 ± 0.0051 & 0.8454 ± 0.0051 & 0.8661 ± 0.0039 & 0.8706 ± 0.0048 & 0.8679 ± 0.0039 & 0.8697 ± 0.0059 & 0.8517 ± 0.0048 \\
\cline{1-10} \cline{2-10}
\multirow[t]{44}{*}{pacs} & \multirow[t]{11}{*}{0} & DANN & 0.2956 ± 0.0118 & 0.3337 ± 0.0150 & 0.3171 ± 0.0079 & 0.3698 ± 0.0179 & 0.4059 ± 0.0192 & 0.4215 ± 0.0124 & 0.3572 ± 0.0140 \\
    &  & DIWA & 0.9405 ± 0.0081 & 0.9346 ± 0.0033 & 0.9512 ± 0.0077 & 0.9551 ± 0.0036 & 0.9473 ± 0.0076 & 0.9444 ± 0.0065 & 0.9455 ± 0.0061 \\
    &  & ERM & 0.8702 ± 0.0043 & 0.8673 ± 0.0042 & 0.8849 ± 0.0068 & 0.9044 ± 0.0059 & 0.9141 ± 0.0072 & 0.9190 ± 0.0037 & 0.8933 ± 0.0053 \\
    &  & NUC\_0.01 & 0.8429 ± 0.0052 & 0.8780 ± 0.0056 & 0.8937 ± 0.0036 & 0.9015 ± 0.0066 & 0.8966 ± 0.0070 & 0.8966 ± 0.0054 & 0.8849 ± 0.0056 \\
    &  & NUC\_0.1 & 0.8273 ± 0.0070 & 0.8702 ± 0.0099 & 0.8839 ± 0.0081 & 0.9024 ± 0.0044 & 0.8976 ± 0.0083 & 0.8937 ± 0.0099 & 0.8792 ± 0.0079 \\
    &  & PN\_B & 0.8810 ± 0.0077 & 0.8878 ± 0.0074 & 0.9239 ± 0.0065 & 0.9190 ± 0.0059 & 0.9307 ± 0.0071 & 0.9288 ± 0.0065 & 0.9119 ± 0.0068 \\
    &  & PN\_B-Y & 0.8849 ± 0.0072 & 0.8868 ± 0.0076 & 0.9190 ± 0.0037 & 0.9180 ± 0.0039 & 0.9337 ± 0.0045 & 0.9346 ± 0.0075 & 0.9128 ± 0.0057 \\
    &  & PN\_B-Y-S-E & 0.9024 ± 0.0044 & 0.9054 ± 0.0043 & 0.9220 ± 0.0046 & 0.9337 ± 0.0077 & 0.9434 ± 0.0061 & 0.9405 ± 0.0047 & 0.9246 ± 0.0053 \\
    &  & PN\_Y & 0.9054 ± 0.0048 & 0.9005 ± 0.0092 & 0.9268 ± 0.0034 & 0.9317 ± 0.0053 & 0.9337 ± 0.0048 & 0.9268 ± 0.0031 & 0.9208 ± 0.0051 \\
    &  & PN\_Y-S & 0.9122 ± 0.0084 & 0.8917 ± 0.0068 & 0.9220 ± 0.0074 & 0.9327 ± 0.0039 & 0.9337 ± 0.0037 & 0.9220 ± 0.0051 & 0.9190 ± 0.0059 \\
    &  & PN\_Y-S-E & 0.9073 ± 0.0034 & 0.9024 ± 0.0067 & 0.9171 ± 0.0094 & 0.9239 ± 0.0067 & 0.9415 ± 0.0041 & 0.9210 ± 0.0086 & 0.9189 ± 0.0065 \\
\cline{2-10}
    & \multirow[t]{11}{*}{1} & DANN & 0.3419 ± 0.0137 & 0.3983 ± 0.0048 & 0.4256 ± 0.0048 & 0.4359 ± 0.0102 & 0.4538 ± 0.0148 & 0.4906 ± 0.0068 & 0.4244 ± 0.0092 \\
    &  & DIWA & 0.8906 ± 0.0098 & 0.9154 ± 0.0067 & 0.9231 ± 0.0072 & 0.9402 ± 0.0045 & 0.9402 ± 0.0038 & 0.9342 ± 0.0089 & 0.9239 ± 0.0068 \\
    &  & ERM & 0.8752 ± 0.0114 & 0.9111 ± 0.0065 & 0.9231 ± 0.0062 & 0.9316 ± 0.0076 & 0.9470 ± 0.0037 & 0.9581 ± 0.0086 & 0.9244 ± 0.0074 \\
    &  & NUC\_0.01 & 0.8436 ± 0.0083 & 0.8581 ± 0.0075 & 0.8897 ± 0.0044 & 0.8974 ± 0.0045 & 0.8906 ± 0.0042 & 0.9179 ± 0.0048 & 0.8829 ± 0.0056 \\
    &  & NUC\_0.1 & 0.8308 ± 0.0046 & 0.8624 ± 0.0044 & 0.8923 ± 0.0076 & 0.8949 ± 0.0086 & 0.9034 ± 0.0068 & 0.9145 ± 0.0030 & 0.8830 ± 0.0058 \\
    &  & PN\_B & 0.9034 ± 0.0064 & 0.9205 ± 0.0064 & 0.9308 ± 0.0067 & 0.9256 ± 0.0026 & 0.9265 ± 0.0028 & 0.9436 ± 0.0046 & 0.9251 ± 0.0049 \\
    &  & PN\_B-Y & 0.9222 ± 0.0056 & 0.9162 ± 0.0064 & 0.9179 ± 0.0095 & 0.9171 ± 0.0032 & 0.9350 ± 0.0031 & 0.9359 ± 0.0076 & 0.9241 ± 0.0059 \\
    &  & PN\_B-Y-S-E & 0.9128 ± 0.0032 & 0.9248 ± 0.0072 & 0.9342 ± 0.0052 & 0.9359 ± 0.0041 & 0.9487 ± 0.0027 & 0.9487 ± 0.0043 & 0.9342 ± 0.0044 \\
    &  & PN\_Y & 0.9068 ± 0.0104 & 0.9282 ± 0.0048 & 0.9231 ± 0.0052 & 0.9359 ± 0.0019 & 0.9308 ± 0.0078 & 0.9487 ± 0.0014 & 0.9289 ± 0.0052 \\
    &  & PN\_Y-S & 0.9162 ± 0.0053 & 0.9342 ± 0.0017 & 0.9265 ± 0.0046 & 0.9427 ± 0.0048 & 0.9368 ± 0.0046 & 0.9556 ± 0.0052 & 0.9353 ± 0.0044 \\
    &  & PN\_Y-S-E & 0.9077 ± 0.0074 & 0.9342 ± 0.0032 & 0.9291 ± 0.0040 & 0.9342 ± 0.0066 & 0.9479 ± 0.0039 & 0.9513 ± 0.0055 & 0.9340 ± 0.0051 \\
\cline{2-10}
    & \multirow[t]{11}{*}{2} & DANN & 0.6431 ± 0.0062 & 0.6311 ± 0.0140 & 0.6862 ± 0.0122 & 0.6862 ± 0.0082 & 0.7186 ± 0.0143 & 0.7138 ± 0.0088 & 0.6798 ± 0.0106 \\
    &  & DIWA & 0.9737 ± 0.0031 & 0.9737 ± 0.0015 & 0.9820 ± 0.0033 & 0.9880 ± 0.0000 & 0.9796 ± 0.0031 & 0.9844 ± 0.0031 & 0.9802 ± 0.0023 \\
    &  & ERM & 0.9533 ± 0.0035 & 0.9569 ± 0.0035 & 0.9653 ± 0.0040 & 0.9677 ± 0.0056 & 0.9677 ± 0.0052 & 0.9593 ± 0.0035 & 0.9617 ± 0.0042 \\
    &  & NUC\_0.01 & 0.9569 ± 0.0064 & 0.9737 ± 0.0045 & 0.9749 ± 0.0055 & 0.9916 ± 0.0031 & 0.9808 ± 0.0022 & 0.9880 ± 0.0019 & 0.9776 ± 0.0039 \\
    &  & NUC\_0.1 & 0.9545 ± 0.0024 & 0.9760 ± 0.0019 & 0.9784 ± 0.0049 & 0.9868 ± 0.0022 & 0.9808 ± 0.0035 & 0.9904 ± 0.0024 & 0.9778 ± 0.0029 \\
    &  & PN\_B & 0.9701 ± 0.0060 & 0.9796 ± 0.0036 & 0.9796 ± 0.0041 & 0.9808 ± 0.0048 & 0.9737 ± 0.0031 & 0.9784 ± 0.0045 & 0.9770 ± 0.0043 \\
    &  & PN\_B-Y & 0.9784 ± 0.0059 & 0.9820 ± 0.0054 & 0.9856 ± 0.0031 & 0.9832 ± 0.0029 & 0.9772 ± 0.0048 & 0.9820 ± 0.0050 & 0.9814 ± 0.0045 \\
    &  & PN\_B-Y-S-E & 0.9796 ± 0.0041 & 0.9772 ± 0.0048 & 0.9808 ± 0.0029 & 0.9796 ± 0.0031 & 0.9784 ± 0.0052 & 0.9880 ± 0.0019 & 0.9806 ± 0.0037 \\
    &  & PN\_Y & 0.9749 ± 0.0029 & 0.9856 ± 0.0031 & 0.9832 ± 0.0040 & 0.9760 ± 0.0033 & 0.9892 ± 0.0012 & 0.9808 ± 0.0022 & 0.9816 ± 0.0028 \\
    &  & PN\_Y-S & 0.9725 ± 0.0024 & 0.9820 ± 0.0050 & 0.9784 ± 0.0062 & 0.9737 ± 0.0045 & 0.9784 ± 0.0024 & 0.9880 ± 0.0019 & 0.9788 ± 0.0037 \\
    &  & PN\_Y-S-E & 0.9641 ± 0.0066 & 0.9760 ± 0.0063 & 0.9820 ± 0.0038 & 0.9904 ± 0.0024 & 0.9784 ± 0.0015 & 0.9832 ± 0.0040 & 0.9790 ± 0.0041 \\
\cline{2-10}
    & \multirow[t]{11}{*}{3} & DANN & 0.6132 ± 0.0038 & 0.6626 ± 0.0069 & 0.7008 ± 0.0071 & 0.6962 ± 0.0120 & 0.7298 ± 0.0049 & 0.7394 ± 0.0091 & 0.6903 ± 0.0073 \\
    &  & DIWA & 0.8718 ± 0.0055 & 0.8896 ± 0.0042 & 0.9170 ± 0.0032 & 0.9074 ± 0.0034 & 0.9115 ± 0.0053 & 0.9160 ± 0.0018 & 0.9022 ± 0.0039 \\
    &  & ERM & 0.8936 ± 0.0039 & 0.8891 ± 0.0030 & 0.9033 ± 0.0052 & 0.9206 ± 0.0057 & 0.9277 ± 0.0046 & 0.9232 ± 0.0041 & 0.9096 ± 0.0044 \\
    &  & NUC\_0.01 & 0.6972 ± 0.0055 & 0.7659 ± 0.0091 & 0.8081 ± 0.0034 & 0.8036 ± 0.0061 & 0.8193 ± 0.0023 & 0.8249 ± 0.0060 & 0.7865 ± 0.0054 \\
    &  & NUC\_0.1 & 0.6987 ± 0.0042 & 0.7603 ± 0.0056 & 0.7969 ± 0.0103 & 0.8107 ± 0.0059 & 0.8249 ± 0.0064 & 0.8275 ± 0.0051 & 0.7865 ± 0.0063 \\
    &  & PN\_B & 0.8427 ± 0.0066 & 0.8718 ± 0.0097 & 0.8840 ± 0.0040 & 0.8967 ± 0.0039 & 0.9033 ± 0.0039 & 0.9013 ± 0.0061 & 0.8833 ± 0.0057 \\
    &  & PN\_B-Y & 0.8601 ± 0.0040 & 0.8636 ± 0.0026 & 0.8947 ± 0.0049 & 0.9018 ± 0.0013 & 0.8901 ± 0.0041 & 0.9069 ± 0.0061 & 0.8862 ± 0.0038 \\
    &  & PN\_B-Y-S-E & 0.8570 ± 0.0033 & 0.8616 ± 0.0057 & 0.8941 ± 0.0030 & 0.8987 ± 0.0035 & 0.9074 ± 0.0061 & 0.9018 ± 0.0055 & 0.8868 ± 0.0045 \\
    &  & PN\_Y & 0.8595 ± 0.0033 & 0.8585 ± 0.0035 & 0.8926 ± 0.0029 & 0.8997 ± 0.0030 & 0.9125 ± 0.0024 & 0.9120 ± 0.0039 & 0.8891 ± 0.0032 \\
    &  & PN\_Y-S & 0.8534 ± 0.0068 & 0.8555 ± 0.0026 & 0.8906 ± 0.0053 & 0.8911 ± 0.0027 & 0.9038 ± 0.0066 & 0.8947 ± 0.0057 & 0.8815 ± 0.0049 \\
    &  & PN\_Y-S-E & 0.8631 ± 0.0047 & 0.8784 ± 0.0057 & 0.8835 ± 0.0049 & 0.8962 ± 0.0045 & 0.9013 ± 0.0025 & 0.8997 ± 0.0051 & 0.8870 ± 0.0046 \\
\cline{1-10} \cline{2-10}
\multirow[t]{44}{*}{terraincognita} & \multirow[t]{11}{*}{0} & DANN & 0.6823 ± 0.0044 & 0.7198 ± 0.0051 & 0.7684 ± 0.0049 & 0.7827 ± 0.0032 & 0.7852 ± 0.0052 & 0.7886 ± 0.0087 & 0.7545 ± 0.0053 \\
    &  & DIWA & 0.8249 ± 0.0058 & 0.8734 ± 0.0037 & 0.9055 ± 0.0062 & 0.9291 ± 0.0025 & 0.9422 ± 0.0076 & 0.9418 ± 0.0020 & 0.9028 ± 0.0046 \\
    &  & ERM & 0.8346 ± 0.0055 & 0.8616 ± 0.0064 & 0.9084 ± 0.0028 & 0.9329 ± 0.0043 & 0.9367 ± 0.0032 & 0.9397 ± 0.0024 & 0.9023 ± 0.0041 \\
    &  & NUC\_0.01 & 0.7928 ± 0.0052 & 0.8329 ± 0.0056 & 0.8730 ± 0.0059 & 0.9105 ± 0.0021 & 0.9219 ± 0.0020 & 0.9291 ± 0.0037 & 0.8767 ± 0.0041 \\
    &  & NUC\_0.1 & 0.7975 ± 0.0110 & 0.8409 ± 0.0054 & 0.8624 ± 0.0039 & 0.9110 ± 0.0051 & 0.9139 ± 0.0036 & 0.9295 ± 0.0044 & 0.8759 ± 0.0055 \\
    &  & PN\_B & 0.8278 ± 0.0058 & 0.8844 ± 0.0045 & 0.9211 ± 0.0011 & 0.9405 ± 0.0018 & 0.9578 ± 0.0009 & 0.9603 ± 0.0044 & 0.9153 ± 0.0031 \\
    &  & PN\_B-Y & 0.8253 ± 0.0049 & 0.8700 ± 0.0049 & 0.9135 ± 0.0049 & 0.9473 ± 0.0033 & 0.9502 ± 0.0023 & 0.9603 ± 0.0035 & 0.9111 ± 0.0040 \\
    &  & PN\_B-Y-S-E & 0.8295 ± 0.0042 & 0.8819 ± 0.0024 & 0.9181 ± 0.0037 & 0.9405 ± 0.0020 & 0.9532 ± 0.0018 & 0.9553 ± 0.0017 & 0.9131 ± 0.0026 \\
    &  & PN\_Y & 0.8392 ± 0.0041 & 0.8819 ± 0.0035 & 0.9131 ± 0.0012 & 0.9540 ± 0.0026 & 0.9519 ± 0.0026 & 0.9608 ± 0.0032 & 0.9168 ± 0.0029 \\
    &  & PN\_Y-S & 0.8287 ± 0.0044 & 0.8747 ± 0.0051 & 0.9165 ± 0.0011 & 0.9502 ± 0.0029 & 0.9506 ± 0.0041 & 0.9578 ± 0.0019 & 0.9131 ± 0.0032 \\
    &  & PN\_Y-S-E & 0.8300 ± 0.0032 & 0.8844 ± 0.0041 & 0.9190 ± 0.0061 & 0.9586 ± 0.0047 & 0.9515 ± 0.0012 & 0.9586 ± 0.0029 & 0.9170 ± 0.0037 \\
\cline{2-10}
    & \multirow[t]{11}{*}{1} & DANN & 0.6875 ± 0.0026 & 0.7294 ± 0.0037 & 0.7760 ± 0.0028 & 0.7690 ± 0.0067 & 0.7727 ± 0.0052 & 0.7729 ± 0.0038 & 0.7512 ± 0.0041 \\
    &  & DIWA & 0.8405 ± 0.0027 & 0.8692 ± 0.0027 & 0.8893 ± 0.0016 & 0.8955 ± 0.0047 & 0.9181 ± 0.0018 & 0.9281 ± 0.0026 & 0.8901 ± 0.0027 \\
    &  & ERM & 0.8351 ± 0.0041 & 0.8643 ± 0.0016 & 0.8916 ± 0.0016 & 0.9064 ± 0.0022 & 0.9341 ± 0.0026 & 0.9300 ± 0.0022 & 0.8936 ± 0.0024 \\
    &  & NUC\_0.01 & 0.7947 ± 0.0033 & 0.8246 ± 0.0038 & 0.8561 ± 0.0030 & 0.8836 ± 0.0021 & 0.8949 ± 0.0030 & 0.8998 ± 0.0016 & 0.8589 ± 0.0028 \\
    &  & NUC\_0.1 & 0.7951 ± 0.0040 & 0.8366 ± 0.0059 & 0.8690 ± 0.0039 & 0.8852 ± 0.0045 & 0.8869 ± 0.0033 & 0.9008 ± 0.0024 & 0.8623 ± 0.0040 \\
    &  & PN\_B & 0.8310 ± 0.0061 & 0.8713 ± 0.0044 & 0.9074 ± 0.0013 & 0.9117 ± 0.0019 & 0.9220 ± 0.0021 & 0.9347 ± 0.0030 & 0.8963 ± 0.0031 \\
    &  & PN\_B-Y & 0.8302 ± 0.0066 & 0.8622 ± 0.0026 & 0.8996 ± 0.0037 & 0.9140 ± 0.0043 & 0.9300 ± 0.0016 & 0.9398 ± 0.0036 & 0.8960 ± 0.0037 \\
    &  & PN\_B-Y-S-E & 0.8267 ± 0.0050 & 0.8637 ± 0.0025 & 0.8922 ± 0.0029 & 0.9156 ± 0.0031 & 0.9296 ± 0.0047 & 0.9368 ± 0.0015 & 0.8941 ± 0.0033 \\
    &  & PN\_Y & 0.8248 ± 0.0036 & 0.8550 ± 0.0047 & 0.8895 ± 0.0021 & 0.9179 ± 0.0040 & 0.9290 ± 0.0011 & 0.9326 ± 0.0037 & 0.8915 ± 0.0032 \\
    &  & PN\_Y-S & 0.8197 ± 0.0053 & 0.8544 ± 0.0031 & 0.8926 ± 0.0015 & 0.9117 ± 0.0037 & 0.9257 ± 0.0023 & 0.9304 ± 0.0026 & 0.8891 ± 0.0031 \\
    &  & PN\_Y-S-E & 0.8230 ± 0.0028 & 0.8706 ± 0.0021 & 0.8834 ± 0.0033 & 0.9166 ± 0.0055 & 0.9324 ± 0.0020 & 0.9347 ± 0.0011 & 0.8935 ± 0.0028 \\
\cline{2-10}
    & \multirow[t]{11}{*}{2} & DANN & 0.5275 ± 0.0066 & 0.6045 ± 0.0061 & 0.6453 ± 0.0065 & 0.6403 ± 0.0081 & 0.6665 ± 0.0056 & 0.6690 ± 0.0043 & 0.6255 ± 0.0062 \\
    &  & DIWA & 0.7264 ± 0.0102 & 0.7909 ± 0.0046 & 0.8040 ± 0.0039 & 0.8458 ± 0.0062 & 0.8499 ± 0.0091 & 0.8872 ± 0.0045 & 0.8174 ± 0.0064 \\
    &  & ERM & 0.7330 ± 0.0112 & 0.7864 ± 0.0084 & 0.8317 ± 0.0043 & 0.8640 ± 0.0044 & 0.8831 ± 0.0055 & 0.8912 ± 0.0029 & 0.8316 ± 0.0061 \\
    &  & NUC\_0.01 & 0.6448 ± 0.0048 & 0.7380 ± 0.0064 & 0.7889 ± 0.0045 & 0.8388 ± 0.0066 & 0.8589 ± 0.0071 & 0.8615 ± 0.0048 & 0.7885 ± 0.0057 \\
    &  & NUC\_0.1 & 0.6534 ± 0.0067 & 0.7345 ± 0.0101 & 0.7950 ± 0.0103 & 0.8368 ± 0.0049 & 0.8615 ± 0.0063 & 0.8680 ± 0.0030 & 0.7915 ± 0.0069 \\
    &  & PN\_B & 0.7521 ± 0.0081 & 0.7945 ± 0.0082 & 0.8247 ± 0.0059 & 0.8443 ± 0.0048 & 0.8675 ± 0.0017 & 0.8811 ± 0.0036 & 0.8274 ± 0.0054 \\
    &  & PN\_B-Y & 0.7436 ± 0.0040 & 0.7884 ± 0.0069 & 0.8327 ± 0.0068 & 0.8630 ± 0.0083 & 0.8670 ± 0.0066 & 0.8922 ± 0.0054 & 0.8312 ± 0.0063 \\
    &  & PN\_B-Y-S-E & 0.7345 ± 0.0063 & 0.7904 ± 0.0058 & 0.8277 ± 0.0027 & 0.8670 ± 0.0063 & 0.8856 ± 0.0047 & 0.8992 ± 0.0047 & 0.8341 ± 0.0051 \\
    &  & PN\_Y & 0.7295 ± 0.0044 & 0.7748 ± 0.0089 & 0.8322 ± 0.0045 & 0.8620 ± 0.0059 & 0.8831 ± 0.0033 & 0.9103 ± 0.0029 & 0.8320 ± 0.0050 \\
    &  & PN\_Y-S & 0.7325 ± 0.0073 & 0.7904 ± 0.0079 & 0.8368 ± 0.0106 & 0.8660 ± 0.0037 & 0.8836 ± 0.0075 & 0.9008 ± 0.0023 & 0.8350 ± 0.0065 \\
    &  & PN\_Y-S-E & 0.7451 ± 0.0070 & 0.7788 ± 0.0039 & 0.8287 ± 0.0046 & 0.8610 ± 0.0084 & 0.8932 ± 0.0060 & 0.8957 ± 0.0044 & 0.8338 ± 0.0057 \\
\cline{2-10}
    & \multirow[t]{11}{*}{3} & DANN & 0.4942 ± 0.0087 & 0.5143 ± 0.0048 & 0.5014 ± 0.0034 & 0.5099 ± 0.0098 & 0.5218 ± 0.0020 & 0.5296 ± 0.0069 & 0.5118 ± 0.0059 \\
    &  & DIWA & 0.7156 ± 0.0030 & 0.7340 ± 0.0052 & 0.8116 ± 0.0023 & 0.8255 ± 0.0030 & 0.8616 ± 0.0036 & 0.8810 ± 0.0030 & 0.8049 ± 0.0034 \\
    &  & ERM & 0.7367 ± 0.0067 & 0.7554 ± 0.0093 & 0.8119 ± 0.0053 & 0.8265 ± 0.0045 & 0.8527 ± 0.0055 & 0.8779 ± 0.0010 & 0.8102 ± 0.0054 \\
    &  & NUC\_0.01 & 0.6442 ± 0.0070 & 0.7061 ± 0.0072 & 0.7687 ± 0.0062 & 0.8122 ± 0.0052 & 0.8337 ± 0.0036 & 0.8456 ± 0.0033 & 0.7684 ± 0.0054 \\
    &  & NUC\_0.1 & 0.6633 ± 0.0061 & 0.7139 ± 0.0055 & 0.7759 ± 0.0069 & 0.8027 ± 0.0046 & 0.8340 ± 0.0025 & 0.8442 ± 0.0053 & 0.7723 ± 0.0051 \\
    &  & PN\_B & 0.7310 ± 0.0068 & 0.7735 ± 0.0060 & 0.8221 ± 0.0049 & 0.8398 ± 0.0062 & 0.8660 ± 0.0029 & 0.8810 ± 0.0074 & 0.8189 ± 0.0057 \\
    &  & PN\_B-Y & 0.7241 ± 0.0069 & 0.7701 ± 0.0024 & 0.8265 ± 0.0038 & 0.8507 ± 0.0054 & 0.8724 ± 0.0058 & 0.8827 ± 0.0041 & 0.8211 ± 0.0047 \\
    &  & PN\_B-Y-S-E & 0.7446 ± 0.0054 & 0.7721 ± 0.0037 & 0.8173 ± 0.0032 & 0.8520 ± 0.0031 & 0.8861 ± 0.0061 & 0.8857 ± 0.0056 & 0.8263 ± 0.0045 \\
    &  & PN\_Y & 0.7357 ± 0.0037 & 0.7748 ± 0.0042 & 0.8126 ± 0.0065 & 0.8500 ± 0.0037 & 0.8680 ± 0.0046 & 0.8847 ± 0.0041 & 0.8210 ± 0.0045 \\
    &  & PN\_Y-S & 0.7391 ± 0.0058 & 0.7568 ± 0.0030 & 0.8184 ± 0.0070 & 0.8463 ± 0.0067 & 0.8694 ± 0.0082 & 0.8816 ± 0.0013 & 0.8186 ± 0.0053 \\
    &  & PN\_Y-S-E & 0.7432 ± 0.0031 & 0.7823 ± 0.0065 & 0.7980 ± 0.0028 & 0.8432 ± 0.0010 & 0.8782 ± 0.0049 & 0.8898 ± 0.0032 & 0.8224 ± 0.0036 \\
\cline{1-10} \cline{2-10}
\multirow[t]{44}{*}{vlcs} & \multirow[t]{11}{*}{0} & DANN & 0.9620 ± 0.0042 & 0.9761 ± 0.0065 & 0.9831 ± 0.0053 & 0.9859 ± 0.0039 & 0.9930 ± 0.0022 & 0.9930 ± 0.0031 & 0.9822 ± 0.0042 \\
    &  & DIWA & 0.9873 ± 0.0052 & 0.9930 ± 0.0039 & 0.9972 ± 0.0028 & 1.0000 ± 0.0000 & 0.9887 ± 0.0053 & 1.0000 ± 0.0000 & 0.9944 ± 0.0029 \\
    &  & ERM & 0.9901 ± 0.0036 & 0.9873 ± 0.0034 & 0.9873 ± 0.0056 & 0.9775 ± 0.0068 & 0.9831 ± 0.0036 & 0.9972 ± 0.0017 & 0.9871 ± 0.0041 \\
    &  & NUC\_0.01 & 1.0000 ± 0.0000 & 1.0000 ± 0.0000 & 1.0000 ± 0.0000 & 1.0000 ± 0.0000 & 1.0000 ± 0.0000 & 0.9944 ± 0.0056 & 0.9991 ± 0.0009 \\
    &  & NUC\_0.1 & 1.0000 ± 0.0000 & 1.0000 ± 0.0000 & 1.0000 ± 0.0000 & 1.0000 ± 0.0000 & 1.0000 ± 0.0000 & 1.0000 ± 0.0000 & 1.0000 ± 0.0000 \\
    &  & PN\_B & 0.9887 ± 0.0036 & 0.9930 ± 0.0022 & 0.9944 ± 0.0026 & 0.9972 ± 0.0017 & 0.9944 ± 0.0026 & 0.9986 ± 0.0014 & 0.9944 ± 0.0024 \\
    &  & PN\_B-Y & 0.9901 ± 0.0017 & 0.9944 ± 0.0014 & 0.9930 ± 0.0022 & 0.9972 ± 0.0017 & 0.9972 ± 0.0017 & 0.9958 ± 0.0017 & 0.9946 ± 0.0018 \\
    &  & PN\_B-Y-S-E & 0.9958 ± 0.0017 & 0.9944 ± 0.0026 & 0.9958 ± 0.0017 & 0.9944 ± 0.0014 & 0.9901 ± 0.0028 & 0.9972 ± 0.0017 & 0.9946 ± 0.0020 \\
    &  & PN\_Y & 0.9958 ± 0.0028 & 0.9915 ± 0.0041 & 0.9915 ± 0.0026 & 0.9901 ± 0.0017 & 0.9986 ± 0.0014 & 0.9972 ± 0.0017 & 0.9941 ± 0.0024 \\
    &  & PN\_Y-S & 0.9901 ± 0.0036 & 0.9845 ± 0.0041 & 0.9944 ± 0.0026 & 0.9930 ± 0.0000 & 0.9986 ± 0.0014 & 0.9915 ± 0.0026 & 0.9920 ± 0.0024 \\
    &  & PN\_Y-S-E & 0.9944 ± 0.0026 & 0.9972 ± 0.0017 & 0.9972 ± 0.0017 & 0.9873 ± 0.0014 & 0.9915 ± 0.0026 & 0.9972 ± 0.0017 & 0.9941 ± 0.0020 \\
\cline{2-10}
    & \multirow[t]{11}{*}{1} & DANN & 0.5429 ± 0.0039 & 0.5526 ± 0.0034 & 0.6293 ± 0.0076 & 0.6391 ± 0.0160 & 0.6429 ± 0.0081 & 0.6368 ± 0.0089 & 0.6073 ± 0.0080 \\
    &  & DIWA & 0.7414 ± 0.0034 & 0.7504 ± 0.0102 & 0.7722 ± 0.0057 & 0.7729 ± 0.0070 & 0.7805 ± 0.0069 & 0.7992 ± 0.0096 & 0.7694 ± 0.0071 \\
    &  & ERM & 0.7519 ± 0.0083 & 0.7263 ± 0.0088 & 0.7549 ± 0.0082 & 0.7586 ± 0.0101 & 0.7707 ± 0.0090 & 0.7609 ± 0.0096 & 0.7539 ± 0.0090 \\
    &  & NUC\_0.01 & 0.7331 ± 0.0117 & 0.7677 ± 0.0088 & 0.7692 ± 0.0094 & 0.7722 ± 0.0070 & 0.7602 ± 0.0038 & 0.7654 ± 0.0104 & 0.7613 ± 0.0085 \\
    &  & NUC\_0.1 & 0.7331 ± 0.0092 & 0.7451 ± 0.0150 & 0.7654 ± 0.0128 & 0.7609 ± 0.0054 & 0.7549 ± 0.0060 & 0.7737 ± 0.0102 & 0.7555 ± 0.0098 \\
    &  & PN\_B & 0.7113 ± 0.0066 & 0.7331 ± 0.0087 & 0.7669 ± 0.0110 & 0.7662 ± 0.0038 & 0.7421 ± 0.0044 & 0.7519 ± 0.0067 & 0.7452 ± 0.0069 \\
    &  & PN\_B-Y & 0.7083 ± 0.0066 & 0.7617 ± 0.0059 & 0.7699 ± 0.0084 & 0.7729 ± 0.0076 & 0.7571 ± 0.0104 & 0.7707 ± 0.0072 & 0.7568 ± 0.0077 \\
    &  & PN\_B-Y-S-E & 0.7248 ± 0.0069 & 0.7511 ± 0.0048 & 0.7767 ± 0.0035 & 0.7564 ± 0.0099 & 0.7481 ± 0.0128 & 0.7609 ± 0.0081 & 0.7530 ± 0.0077 \\
    &  & PN\_Y & 0.7346 ± 0.0050 & 0.7797 ± 0.0130 & 0.7992 ± 0.0116 & 0.7677 ± 0.0129 & 0.7519 ± 0.0059 & 0.7842 ± 0.0102 & 0.7695 ± 0.0098 \\
    &  & PN\_Y-S & 0.7203 ± 0.0059 & 0.7782 ± 0.0098 & 0.7714 ± 0.0077 & 0.7669 ± 0.0102 & 0.7466 ± 0.0112 & 0.7534 ± 0.0061 & 0.7561 ± 0.0085 \\
    &  & PN\_Y-S-E & 0.7256 ± 0.0086 & 0.7774 ± 0.0129 & 0.7774 ± 0.0076 & 0.7571 ± 0.0137 & 0.7654 ± 0.0165 & 0.7511 ± 0.0069 & 0.7590 ± 0.0110 \\
\cline{2-10}
    & \multirow[t]{11}{*}{2} & DANN & 0.7927 ± 0.0080 & 0.8012 ± 0.0114 & 0.7817 ± 0.0060 & 0.7976 ± 0.0056 & 0.7854 ± 0.0053 & 0.8091 ± 0.0126 & 0.7946 ± 0.0081 \\
    &  & DIWA & 0.8201 ± 0.0075 & 0.8073 ± 0.0068 & 0.8189 ± 0.0039 & 0.8146 ± 0.0077 & 0.8049 ± 0.0066 & 0.8104 ± 0.0080 & 0.8127 ± 0.0067 \\
    &  & ERM & 0.8104 ± 0.0077 & 0.8268 ± 0.0046 & 0.8293 ± 0.0048 & 0.8152 ± 0.0105 & 0.8299 ± 0.0078 & 0.8311 ± 0.0124 & 0.8238 ± 0.0080 \\
    &  & NUC\_0.01 & 0.8067 ± 0.0100 & 0.8213 ± 0.0050 & 0.8262 ± 0.0043 & 0.8329 ± 0.0079 & 0.8140 ± 0.0027 & 0.8189 ± 0.0079 & 0.8200 ± 0.0063 \\
    &  & NUC\_0.1 & 0.8006 ± 0.0072 & 0.8262 ± 0.0061 & 0.8354 ± 0.0042 & 0.8274 ± 0.0091 & 0.8220 ± 0.0058 & 0.8341 ± 0.0059 & 0.8243 ± 0.0064 \\
    &  & PN\_B & 0.7945 ± 0.0067 & 0.8030 ± 0.0055 & 0.8049 ± 0.0093 & 0.8152 ± 0.0033 & 0.8128 ± 0.0059 & 0.8073 ± 0.0047 & 0.8063 ± 0.0059 \\
    &  & PN\_B-Y & 0.7823 ± 0.0100 & 0.7848 ± 0.0101 & 0.7915 ± 0.0030 & 0.8171 ± 0.0057 & 0.8165 ± 0.0054 & 0.8104 ± 0.0095 & 0.8004 ± 0.0073 \\
    &  & PN\_B-Y-S-E & 0.8073 ± 0.0095 & 0.7970 ± 0.0051 & 0.7957 ± 0.0041 & 0.8067 ± 0.0058 & 0.7963 ± 0.0050 & 0.8165 ± 0.0113 & 0.8033 ± 0.0068 \\
    &  & PN\_Y & 0.7982 ± 0.0118 & 0.7933 ± 0.0049 & 0.8073 ± 0.0053 & 0.8183 ± 0.0053 & 0.8079 ± 0.0042 & 0.8055 ± 0.0089 & 0.8051 ± 0.0067 \\
    &  & PN\_Y-S & 0.7963 ± 0.0064 & 0.7866 ± 0.0059 & 0.8067 ± 0.0059 & 0.8030 ± 0.0062 & 0.8110 ± 0.0058 & 0.8293 ± 0.0042 & 0.8055 ± 0.0057 \\
    &  & PN\_Y-S-E & 0.7957 ± 0.0062 & 0.7939 ± 0.0104 & 0.8024 ± 0.0090 & 0.8073 ± 0.0095 & 0.8213 ± 0.0074 & 0.8244 ± 0.0101 & 0.8075 ± 0.0088 \\
\cline{2-10}
    & \multirow[t]{11}{*}{3} & DANN & 0.5018 ± 0.0121 & 0.5302 ± 0.0022 & 0.5846 ± 0.0061 & 0.5840 ± 0.0012 & 0.5976 ± 0.0075 & 0.5716 ± 0.0037 & 0.5616 ± 0.0055 \\
    &  & DIWA & 0.8491 ± 0.0095 & 0.8728 ± 0.0047 & 0.8550 ± 0.0028 & 0.8651 ± 0.0039 & 0.8550 ± 0.0028 & 0.8580 ± 0.0048 & 0.8592 ± 0.0047 \\
    &  & ERM & 0.8604 ± 0.0069 & 0.8728 ± 0.0129 & 0.8722 ± 0.0036 & 0.8663 ± 0.0077 & 0.8787 ± 0.0066 & 0.8722 ± 0.0049 & 0.8704 ± 0.0071 \\
    &  & NUC\_0.01 & 0.8456 ± 0.0045 & 0.8645 ± 0.0042 & 0.8817 ± 0.0021 & 0.8828 ± 0.0093 & 0.8846 ± 0.0099 & 0.8716 ± 0.0074 & 0.8718 ± 0.0062 \\
    &  & NUC\_0.1 & 0.8467 ± 0.0071 & 0.8686 ± 0.0050 & 0.8757 ± 0.0039 & 0.8864 ± 0.0064 & 0.8947 ± 0.0047 & 0.8751 ± 0.0068 & 0.8746 ± 0.0056 \\
    &  & PN\_B & 0.8609 ± 0.0047 & 0.8556 ± 0.0067 & 0.8740 ± 0.0050 & 0.8763 ± 0.0071 & 0.8657 ± 0.0061 & 0.8609 ± 0.0078 & 0.8656 ± 0.0062 \\
    &  & PN\_B-Y & 0.8621 ± 0.0052 & 0.8556 ± 0.0044 & 0.8722 ± 0.0065 & 0.8675 ± 0.0076 & 0.8651 ± 0.0123 & 0.8734 ± 0.0029 & 0.8660 ± 0.0065 \\
    &  & PN\_B-Y-S-E & 0.8728 ± 0.0039 & 0.8550 ± 0.0049 & 0.8574 ± 0.0055 & 0.8627 ± 0.0049 & 0.8680 ± 0.0058 & 0.8651 ± 0.0061 & 0.8635 ± 0.0052 \\
    &  & PN\_Y & 0.8521 ± 0.0064 & 0.8781 ± 0.0054 & 0.8911 ± 0.0025 & 0.8598 ± 0.0050 & 0.8722 ± 0.0044 & 0.8769 ± 0.0056 & 0.8717 ± 0.0049 \\
    &  & PN\_Y-S & 0.8669 ± 0.0085 & 0.8686 ± 0.0050 & 0.8710 ± 0.0091 & 0.8621 ± 0.0060 & 0.8805 ± 0.0070 & 0.8669 ± 0.0068 & 0.8693 ± 0.0071 \\
    &  & PN\_Y-S-E & 0.8633 ± 0.0037 & 0.8692 ± 0.0041 & 0.8692 ± 0.0090 & 0.8615 ± 0.0059 & 0.8633 ± 0.0081 & 0.8746 ± 0.0030 & 0.8669 ± 0.0057 \\
\cline{1-10} \cline{2-10}
\bottomrule
\end{tabular}

==> figures/6_uda.tex <==
\begin{tabular}{lllllllllllllllllllll}
\toprule
 & \multicolumn{5}{c}{OfficeHome} & \multicolumn{5}{c}{PACS} & \multicolumn{5}{c}{TerrainCognita} & \multicolumn{5}{c}{VLCS} \\
 & A & C & P & R & \textbf{Mean} 
 & A & C & P & S & \textbf{Mean}  
 & L100 & L38 & L43 & L46 & \textbf{Mean} 
 & C & L & S & V & \textbf{Mean}  \\
\midrule
DANN & 0.6091 & 0.0297 & 0.6599 & 0.7408 & 0.5099 & 0.1463 & 0.1026 & 0.6707 & 0.2112 & 0.2827 & 0.0886 & 0.0770 & 0.2040 & 0.2806 & 0.1626 & 0.9437 & 0.3636 & 0.4006 & 0.4438 & 0.5379 \\
DIWA & 0.6914 & 0.5767 & 0.7838 & 0.7982 & 0.7125 & 0.9024 & 0.8162 & 0.9880 & 0.8244 & \textbf{0.8828} & 0.5781 & 0.4517 & 0.5995 & 0.4354 & 0.5162 & 0.9718 & 0.6014 & 0.7350 & 0.8047 & 0.7782 \\
ERM & 0.6914 & 0.5240 & 0.7793 & 0.8211 & 0.7039 & 0.8244 & 0.7906 & 0.9641 & 0.8270 & 0.8515 & 0.5190 & 0.4415 & 0.5693 & 0.3861 & 0.4789 & 0.9718 & 0.6503 & 0.7098 & 0.8136 & 0.7864 \\
NUC-0.01 & 0.6996 & 0.5446 & 0.8018 & 0.8119 & 0.7145 & 0.8244 & 0.7521 & 0.9820 & 0.7888 & 0.8368 & 0.2025 & 0.4138 & 0.5516 & 0.2177 & 0.3464 & 0.3169 & 0.6692 & 0.7652 & 0.1391 & 0.4726 \\
NUC-0.1 & 0.7284 & 0.5423 & 0.7995 & 0.8188 & 0.7223 & 0.8195 & 0.8120 & 0.9880 & 0.7990 & 0.8546 & 0.6181 & 0.4969 & 0.6121 & 0.2177 & 0.4862 & 0.9789 & 0.6842 & 0.7287 & 0.8077 & \textbf{0.7999} \\
PN-Y & 0.7243 & 0.4920 & 0.8063 & 0.8417 & 0.7161 & 0.7707 & 0.8120 & 0.9641 & 0.7150 & 0.8154 & 0.5570 & 0.5277 & 0.5340 & 0.4762 & 0.5237 & 0.9789 & 0.5594 & 0.7382 & 0.8166 & 0.7733 \\
PN-Y-S & 0.7284 & 0.5057 & 0.8108 & 0.8486 & \textbf{0.7234} & 0.7659 & 0.8120 & 0.9641 & 0.6997 & 0.8104 & 0.5612 & 0.5277 & 0.5290 & 0.4728 & 0.5227 & 0.9859 & 0.5594 & 0.7382 & 0.8343 & 0.7795 \\
\bottomrule
\end{tabular}


==> figures/6_uda_back.tex <==
\begin{tabular}{lllllllllllllllllllll}
\toprule
 & \multicolumn{5}{c|}{OfficeHome} & \multicolumn{5}{|c|}{PACS} & \multicolumn{5}{|c|}{TerrainCognita} & \multicolumn{5}{|c}{VLCS} \\
 & 
    \multicolumn{1}{c}{0} & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{0} &
    \multicolumn{1}{|c}{0} & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{0} &
    \multicolumn{1}{|c}{0} & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{0} &
    \multicolumn{1}{|c}{0} & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{0} \\
\midrule
DANN & 0.6091 & 0.0297 & 0.6599 & 0.7408 & 0.5099 & 0.1463 & 0.1026 & 0.6707 & 0.2112 & 0.2827 & 0.0886 & 0.0770 & 0.2040 & 0.2806 & 0.1626 & 0.9437 & 0.3636 & 0.4006 & 0.4438 & 0.5379 \\
DIWA & 0.6914 & 0.5767 & 0.7838 & 0.7982 & 0.7125 & 0.9024 & 0.8162 & 0.9880 & 0.8244 & \textbf{0.8828} & 0.5781 & 0.4517 & 0.5995 & 0.4354 & 0.5162 & 0.9718 & 0.6014 & 0.7350 & 0.8047 & 0.7782 \\
ERM & 0.6914 & 0.5240 & 0.7793 & 0.8211 & 0.7039 & 0.8244 & 0.7906 & 0.9641 & 0.8270 & 0.8515 & 0.5190 & 0.4415 & 0.5693 & 0.3861 & 0.4789 & 0.9718 & 0.6503 & 0.7098 & 0.8136 & 0.7864 \\
NUC-0.01 & 0.6996 & 0.5446 & 0.8018 & 0.8119 & 0.7145 & 0.8244 & 0.7521 & 0.9820 & 0.7888 & 0.8368 & 0.2025 & 0.4138 & 0.5516 & 0.2177 & 0.3464 & 0.3169 & 0.6692 & 0.7652 & 0.1391 & 0.4726 \\
NUC-0.1 & 0.7284 & 0.5423 & 0.7995 & 0.8188 & 0.7223 & 0.8195 & 0.8120 & 0.9880 & 0.7990 & 0.8546 & 0.6181 & 0.4969 & 0.6121 & 0.2177 & 0.4862 & 0.9789 & 0.6842 & 0.7287 & 0.8077 & \textbf{0.7999} \\
PN-Y & 0.7243 & 0.4920 & 0.8063 & 0.8417 & 0.7161 & 0.7707 & 0.8120 & 0.9641 & 0.7150 & 0.8154 & 0.5570 & 0.5277 & 0.5340 & 0.4762 & 0.5237 & 0.9789 & 0.5594 & 0.7382 & 0.8166 & 0.7733 \\
PN-Y-S & 0.7284 & 0.5057 & 0.8108 & 0.8486 & \textbf{0.7234} & 0.7659 & 0.8120 & 0.9641 & 0.6997 & 0.8104 & 0.5612 & 0.5277 & 0.5290 & 0.4728 & 0.5227 & 0.9859 & 0.5594 & 0.7382 & 0.8343 & 0.7795 \\
PN-Y-S-E & 0.7160 & 0.5034 & 0.8086 & 0.8463 & 0.7186 & 0.7756 & 0.8120 & 0.9641 & 0.6921 & 0.8109 & 0.5675 & 0.5246 & 0.5365 & 0.4779 & \textbf{0.5266} & 0.9789 & 0.5594 & 0.7382 & 0.8373 & 0.7784 \\
\bottomrule
\end{tabular}


==> figures/6_uda_with_err.tex <==
\begin{tabular}{lllllll}
    \toprule
     &  & 0 & 1 & 2 & 3 & mean \\
    dataset.name & hue &  &  &  &  &  \\
    \midrule
    \multirow[t]{8}{*}{OfficeHome} & DANN & 0.6091 ± 0.0000 & 0.0297 ± 0.0000 & 0.6599 ± 0.0000 & 0.7408 ± 0.0000 & 0.5099 ± 0.0000 \\
     & DIWA & 0.6914 ± 0.0000 & \textbf{0.5767 ± 0.0000} & 0.7838 ± 0.0000 & 0.7982 ± 0.0000 & 0.7125 ± 0.0000 \\
     & ERM & 0.6914 ± 0.0000 & 0.5240 ± 0.0000 & 0.7793 ± 0.0000 & 0.8211 ± 0.0000 & 0.7039 ± 0.0000 \\
     & NUC-0.01 & 0.6996 ± 0.0000 & 0.5423 ± 0.0000 & 0.8018 ± 0.0000 & 0.8119 ± 0.0000 & 0.7139 ± 0.0000 \\
     & NUC-0.1 & \textbf{0.7284 ± 0.0000} & 0.5400 ± 0.0000 & 0.8018 ± 0.0000 & 0.8188 ± 0.0000 & 0.7223 ± 0.0000 \\
     & PN-y & 0.7243 ± 0.0000 & 0.4920 ± 0.0000 & 0.8063 ± 0.0000 & 0.8417 ± 0.0000 & 0.7161 ± 0.0000 \\
     & PN-Y-s & \textbf{0.7284 ± 0.0000} & 0.5057 ± 0.0000 & \textbf{0.8108 ± 0.0000} & \textbf{0.8486 ± 0.0000} & \textbf{0.7234 ± 0.0000} \\
     & PN-Y-S-E & 0.7210 ± 0.0015 & 0.4998 ± 0.0019 & 0.8077 ± 0.0015 & 0.8468 ± 0.0015 & 0.7188 ± 0.0016 \\
    \cline{1-7}
    \multirow[t]{8}{*}{PACS} & DANN & 0.1463 ± 0.0000 & 0.1026 ± 0.0000 & 0.6707 ± 0.0000 & 0.2112 ± 0.0000 & 0.2827 ± 0.0000 \\
     & DIWA & \textbf{0.9073 ± 0.0000} & 0.8120 ± 0.0000 & \textbf{0.9880 ± 0.0000} & 0.8244 ± 0.0000 & \textbf{0.8829 ± 0.0000} \\
     & ERM & 0.8244 ± 0.0000 & 0.7863 ± 0.0000 & 0.9820 ± 0.0000 & \textbf{0.8270 ± 0.0000} & 0.8549 ± 0.0000 \\
     & NUC-0.01 & 0.8293 ± 0.0000 & 0.7906 ± 0.0000 & 0.9760 ± 0.0000 & 0.7863 ± 0.0000 & 0.8455 ± 0.0000 \\
     & NUC-0.1 & 0.8780 ± 0.0000 & 0.7991 ± 0.0000 & 0.9760 ± 0.0000 & 0.8041 ± 0.0000 & 0.8643 ± 0.0000 \\
     & PN-y & 0.7707 ± 0.0000 & \textbf{0.8162 ± 0.0000} & 0.9641 ± 0.0000 & 0.7150 ± 0.0000 & 0.8165 ± 0.0000 \\
     & PN-Y-s & 0.7668 ± 0.0010 & 0.8077 ± 0.0000 & 0.9641 ± 0.0000 & 0.6997 ± 0.0000 & 0.8096 ± 0.0002 \\
     & PN-Y-S-E & 0.7766 ± 0.0018 & 0.8085 ± 0.0009 & 0.9653 ± 0.0012 & 0.6972 ± 0.0024 & 0.8119 ± 0.0016 \\
    \cline{1-7}
    \multirow[t]{8}{*}{TerraIncognita} & DANN & 0.0907 ± 0.0000 & 0.0770 ± 0.0000 & 0.2040 ± 0.0000 & 0.2806 ± 0.0000 & 0.1631 ± 0.0000 \\
     & DIWA & 0.5781 ± 0.0000 & 0.4517 ± 0.0000 & 0.5995 ± 0.0000 & 0.4354 ± 0.0000 & 0.5162 ± 0.0000 \\
     & ERM & 0.5190 ± 0.0000 & 0.4415 ± 0.0000 & 0.5617 ± 0.0000 & 0.3861 ± 0.0000 & 0.4771 ± 0.0000 \\
     & NUC-0.01 & 0.5401 ± 0.0000 & 0.4138 ± 0.0000 & 0.5516 ± 0.0000 & 0.3316 ± 0.0000 & 0.4593 ± 0.0000 \\
     & NUC-0.1 & \textbf{0.6203 ± 0.0000} & 0.4988 ± 0.0002 & \textbf{0.6096 ± 0.0000} & 0.4116 ± 0.0000 & \textbf{0.5350 ± 0.0001} \\
     & PN-y & 0.5570 ± 0.0000 & \textbf{0.5277 ± 0.0000} & 0.5340 ± 0.0000 & 0.4762 ± 0.0000 & 0.5237 ± 0.0000 \\
     & PN-Y-s & 0.5591 ± 0.0000 & \textbf{0.5277 ± 0.0000} & 0.5290 ± 0.0000 & 0.4728 ± 0.0000 & 0.5221 ± 0.0000 \\
     & PN-Y-S-E & 0.5641 ± 0.0016 & 0.5253 ± 0.0009 & 0.5345 ± 0.0027 & \textbf{0.4765 ± 0.0018} & 0.5251 ± 0.0017 \\
    \cline{1-7}
    \multirow[t]{8}{*}{VLCS} & DANN & 0.9437 ± 0.0000 & 0.3636 ± 0.0000 & 0.4006 ± 0.0000 & 0.4438 ± 0.0000 & 0.5379 ± 0.0000 \\
     & DIWA & 0.9718 ± 0.0000 & 0.6014 ± 0.0000 & 0.7350 ± 0.0000 & 0.8047 ± 0.0000 & 0.7782 ± 0.0000 \\
     & ERM & 0.9718 ± 0.0000 & \textbf{0.6503 ± 0.0000} & 0.7098 ± 0.0000 & 0.8112 ± 0.0006 & 0.7858 ± 0.0001 \\
     & NUC-0.01 & 0.9789 ± 0.0000 & 0.6364 ± 0.0000 & 0.7382 ± 0.0000 & 0.8018 ± 0.0000 & 0.7888 ± 0.0000 \\
     & NUC-0.1 & 0.9789 ± 0.0000 & 0.6364 ± 0.0000 & \textbf{0.7476 ± 0.0000} & 0.8018 ± 0.0000 & \textbf{0.7912 ± 0.0000} \\
     & PN-y & 0.9789 ± 0.0000 & 0.5594 ± 0.0000 & 0.7382 ± 0.0000 & 0.8343 ± 0.0000 & 0.7777 ± 0.0000 \\
     & PN-Y-s & \textbf{0.9859 ± 0.0000} & 0.5594 ± 0.0000 & 0.7382 ± 0.0000 & 0.8314 ± 0.0000 & 0.7787 ± 0.0000 \\
     & PN-Y-S-E & 0.9817 ± 0.0017 & 0.5650 ± 0.0026 & 0.7344 ± 0.0023 & \textbf{0.8367 ± 0.0011} & 0.7794 ± 0.0019 \\
    \cline{1-7}
    \bottomrule
    \end{tabular}
    
